LinkedIn Salary: A System for Secure Collection and Presentation of Structured Compensation Insights to Job Seekers

Online professional social networks such as LinkedIn have enhanced the ability of job seekers to discover and assess career opportunities, and the ability of job providers to discover and assess potential candidates. For most job seekers, salary (or broadly compensation) is a crucial consideration in choosing a new job. At the same time, job seekers face challenges in learning the compensation associated with different jobs, given the sensitive nature of compensation data and the dearth of reliable sources containing compensation data. Towards the goal of helping the world's professionals optimize their earning potential through salary transparency, we present LinkedIn Salary, a system for collecting compensation information from LinkedIn members and providing compensation insights to job seekers. We present the overall design and architecture, and describe the key components needed for the secure collection, de-identification, and processing of compensation data, focusing on the unique challenges associated with privacy and security. We perform an experimental study with more than one year of compensation submission history data collected from over 1.5 million LinkedIn members, thereby demonstrating the tradeoffs between privacy and modeling needs. We also highlight the lessons learned from the production deployment of this system at LinkedIn.

==> Makefile <==
RCSFLAGS= -l
MAIN=linkedinSalaryArchitecture

TEXPARTS= *.tex 

BIBPARTS= *.bib
POSTSCRIPT= dvips -P cmz -t letter  #dvips -f
#POSTSCRIPT= dvips -P cmz -t a4  #dvips -f
PS2PDF= ps2pdf -dPDFSETTINGS=/prepress -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true 
FIGPARTS = FIG
PDFLATEX=pdflatex

# target: all - Compile ps and pdf
all: $(MAIN).pdf
#all: $(MAIN).dvi
#	$(POSTSCRIPT) -o $(MAIN).ps $(MAIN).dvi
#	$(PS2PDF) $(MAIN).ps $(MAIN).pdf

# target: help - Display callable targets.
help:
	egrep "^# target:" Makefile

$(MAIN).pdf:
	$(PDFLATEX) $(MAIN).tex && bibtex $(MAIN) && $(PDFLATEX) $(MAIN).tex && $(PDFLATEX) $(MAIN).tex

$(MAIN).dvi: $(TEXPARTS) $(BIBPARTS)
	latex $(MAIN).tex
	bibtex $(MAIN)
	latex $(MAIN).tex
	latex $(MAIN).tex

# target: clean - Clean all intermediate compilation products
clean:
	\rm -f *.dvi $(MAIN).ps $(MAIN).pdf *.bbl *.aux *.log *.blg *.toc $(MAIN).tar* $(MAIN).tar.gz *~ *.bak

# target: tar - Create a gz tarball with all tex, bib, figures, and makefile
tar:
	tar cvfh $(MAIN).tar Makefile $(TEXPARTS) $(BIBPARTS) *.eps
	gzip $(MAIN).tar

